Performance optimizations for porting the openQ$^\star$D package to GPUs

OpenQ$^\star$D code has been used by the RC$^\star$ collaboration for the generation of fully dynamical QCD+QED gauge configurations with C$^\star$ boundary conditions. In this talk, optimization of solvers provided with the openQ$^\star$D package relevant for porting the code on GPU-accelerated supercomputing platforms is discussed. We present the analysis of the current implementations of the GCR solver preconditioned with Schwarz alternating procedure for ill-conditioned Dirac-operators. With the goal of enabling support for GPUs from various vendors, a novel method of adaptive CPU/GPU-hybrid implementation is proposed.

==> include/colors.tex <==
%
% genertated by ./compile.py
%

\definecolor{codegreen}{RGB}{0, 153, 0}
\definecolor{codegray}{RGB}{127, 127, 127}
\definecolor{codeblue}{RGB}{102, 214, 237}
\definecolor{codekeyword}{RGB}{249, 36, 114}
\definecolor{codecomment}{RGB}{127, 127, 127}
\definecolor{backcolor}{RGB}{242, 242, 235}
\definecolor{linkcolor}{RGB}{102, 0, 0}
\definecolor{corange}{RGB}{255, 70, 0}
\definecolor{cyellow}{RGB}{209, 153, 0}
\definecolor{cblue}{RGB}{64, 128, 255}
\definecolor{cbrown}{RGB}{153, 102, 51}
\definecolor{cpink}{RGB}{255, 0, 255}
\definecolor{cred}{RGB}{255, 64, 0}
\definecolor{cgreen}{RGB}{0, 191, 0}
\definecolor{clightblue}{RGB}{191, 217, 255}
\definecolor{cturquois}{RGB}{0, 255, 255}
\definecolor{cpurple}{RGB}{128, 0, 255}
\definecolor{clightgreen}{RGB}{175, 255, 175}
\definecolor{clightpink}{RGB}{255, 175, 255}
\definecolor{cdarkblue}{RGB}{0, 0, 255}
\definecolor{cdarkred}{RGB}{255, 0, 0}
\definecolor{cdarkgreen}{RGB}{0, 255, 0}

